Optimizing Bipedal Maneuvers of Single Rigid-Body Models for Reinforcement Learning

In this work, we propose a method to generate reduced-order model reference trajectories for general classes of highly dynamic maneuvers for bipedal robots for use in sim-to-real reinforcement learning. Our approach is to utilize a single rigid-body model (SRBM) to optimize libraries of trajectories offline to be used as expert references in the reward function of a learned policy. This method translates the model's dynamically rich rotational and translational behaviour to a full-order robot model and successfully transfers to real hardware. The SRBM's simplicity allows for fast iteration and refinement of behaviors, while the robustness of learning-based controllers allows for highly dynamic motions to be transferred to hardware. % Within this work we introduce a set of transferability constraints that amend the SRBM dynamics to actual bipedal robot hardware, our framework for creating optimal trajectories for dynamic stepping, turning maneuvers and jumps as well as our approach to integrating reference trajectories to a reinforcement learning policy. Within this work we introduce a set of transferability constraints that amend the SRBM dynamics to actual bipedal robot hardware, our framework for creating optimal trajectories for a variety of highly dynamic maneuvers as well as our approach to integrating reference trajectories for a high-speed running reinforcement learning policy. We validate our methods on the bipedal robot Cassie on which we were successfully able to demonstrate highly dynamic grounded running gaits up to 3.0 m/s.

==> table.tex <==
\begin{table}[!ht]
\centering
\caption{Paper Reading Status.}
\label{tab:reading}
\begin{tabular}{l V{3} l}
\textbf{Status} & \textbf{Papers} \\ \hline \Cline{3pt}{1-2}
\textbf{Will read.} & \cite{Agha-mohammadi2013,Bai2011,Beynier2005,Boutilier1999,Boutilier2000,Cimatti2015,Clark-Turner2017,Ding2011,Feng2004,Gerevini2002,Guestrin2003,Marecki2007,Micheli2015,Nayyar2013,Ono2013,Porta2006,Sanner2009,Toussaint2006} \\ 
\textbf{Skimmed, but will revisit.} & \cite{Amato2015a,Dibangoye2013,Dibangoye2016,Lahijanian2012,Oliehoek2008a,Oliehoek2012,Omidshafiei2016} \\ 
\textbf{Read, but will revisit.} & \cite{Amato2009b,Kumar2010b,Oliehoek2016,Omidshafiei2017,Seuken2008} \\ 
\textbf{Skimmed and will not revisit.} & \cite{Amato2015b,Oliehoek2013} \\ 
\textbf{Read and will not revisit.} & \cite{Amato2013,Amato2014,Amato2016,Beaudry2010a,Beaudry2010b,Beaudry2012,Bresina2002,Buehler2014,Dukeman2017a,Hoang2017,Hoey1999,Marcon2017,Oliehoek2017,Sanner2010a,Sen2013,Sen2015a,Sen2015b,Service2010,Service2011,Service2011a,Service2014,Vig2005,Vig2006,Vig2006a,Vig2007,Witwicki2017} \\ 
\textbf{Abstract/Intro read and will not revisit.} & \cite{Abdallah2004,Alterovitz2016,Amato2007a,Amato2007b,Amato2009,Amato2010a,Amato2010b,Aras2007,Athans1971,Auer2002,Barto1995,Beaudry2011,Becker2004,Benton2012,Bernardini2017,Bernstein2002,Bernstein2005,Bernstein2009,Bertsekas1996,Bigelow2017,Blum1997,Blum2000,Bonet2003,Bose2009,Boularias2008,Boutilier2001,Brown2017,Bryce2015,Buffet2009,Carlin2008,Cashmore2015,Cashmore2015a,Chen2006,Cimatti2018,Claessen2011,Cole2015,Coles2008,Coles2009,Coles2009a,Coles2010,Coles2011,Coles2012,Coles2012a,Cushing2007,Dang2004,Davidson1987,Dennett1991,Dibangoye2009,Dibangoye2014a,Dibangoye2014b,Dimopoulos2012,Dinkla2012,Do2014,Dor1999,Drougard2014,Dudek1996,Dukeman2017,Durfee2013,Dvorak2014,Edelkamp2002,Eker2010,Eker2011,Eker2012,Eker2013,Emery-Montemerlo2004,Erdmann1988,Eyerich2012,Eyerich2014,Farinelli2004,Fox2003,Gaston2005,Geramifard2011,Gerkey2002,Gerkey2004,Ghallab1994,Ghallab2004,Ghallab2016,Goldman2004,Guestrin2001,Guestrin2002,Gursoy1963,Halsey2004,Han2017,Hansen2004,Haque2009,Haslum2014,Hauskrecht1998,Havre2002,Helmert2006,Hoffmann2001,Jimenez2015,Junghanns1997,Junghanns2001,Kaelbling1998,Kautz1992,Keller2012,Keller2013,Kleinberg1999,Kocsis2006,Koes2005,Kolobov2012,Kolobov2012a,Kovacs2012,Krautz1996,Kumar2010a,Kurniawati2008,Kurzweil2013,Kushmerick1994,Kvarnstrom2000,Kvarnstrom2011,Laborie1995,Lagoudakis2004,Lemaire2004,Levesque1998,Lewis2012,Little2005,Liu2014,Liu2016,Long2003,Long2003a,Luo2012,Mausam2008,Mausam2012,McDermott1998,Messias2013,Messias2014,Meyer2009,Meyer2010,Minsky2006,Muise2012,Muise2015,Nair2003,Newell1959,Nilsson1970,Nilsson1980,Oliehoek2008b,Oliehoek2008c,Oliehoek2009a,Oliehoek2010,Olsen2011,Omidshafiei2015,Ong2010,Pajarinen2011a,Pajarinen2011b,Pajarinen2013,Pednault1989,Penberthy1992,Penberthy1994,Petrik2007,Poupart2005,Quigley2009,Raghavan2011,Rahwan2008,Rankooh2015,Ren2008,Rohanimanesh2001,Rothkopf1998,Russell2009,Sacerdoti1975,Sagan1995,Sandholm1999,Sanner2010b,Sanner2011,Sapena2013,Sapena2014,Sariel-Talay2011,Sarvapali2010,Scheepens2011,Searle1980,Selassie2011,Sen2015c,Service2009,Shehory1998,Shiroma2009,Silver2010,Sim2008,Smith1999,Smith2004,Smith2008,Somani2013,Spaan2005,Spaan2011,Steinmetz2016,Sujit2008,Sun2013,Sutton1998,Sutton1999,Sven2007a,Sven2007b,Szer2005a,Szer2005b,Szer2006,Takes2008,Tominski2012,Torralba2014,Tosic2005,Ure2012,Vallati2015,Varakantham2007,Vidal1996,Vidal2004,Vidal2011,Vidal2014,Wagner2011,Watkins2017,Weerdt2007,Winograd1971,Wu2010,Wu2013,Xia2004,Xu2008,Yoon2007,Yoon2008,Yoon2010,Younes2002,Younes2004a,Younes2004b,Younes2004c,Zahra2012,Zhang2010,Zhao2012,Zitzler1999,erol1992,gupta1992} \\ 
\end{tabular}
\end{table}

